Drawing a Map of Elections

Our main contribution is the introduction of the map of elections framework. A map of elections consists of three main elements: (1) a dataset of elections (i.e., collections of ordinal votes over given sets of candidates), (2) a way of measuring similarities between these elections, and (3) a representation of the elections in the 2D Euclidean space as points, so that the more similar two elections are, the closer are their points. In our maps, we mostly focus on datasets of synthetic elections, but we also show an example of a map over real-life ones. To measure similarities, we would have preferred to use, e.g., the isomorphic swap distance, but this is infeasible due to its high computational complexity. Hence, we propose polynomial-time computable positionwise distance and use it instead. Regarding the representations in 2D Euclidean space, we mostly use the Kamada-Kawai algorithm, but we also show two alternatives. We develop the necessary theoretical results to form our maps and argue experimentally that they are accurate and credible. Further, we show how coloring the elections in a map according to various criteria helps in analyzing results of a number of experiments. In particular, we show colorings according to the scores of winning candidates or committees, running times of ILP-based winner determination algorithms, and approximation ratios achieved by particular algorithms.

==> images/Condorcet/condFreq.tex <==
% This file was created by tikzplotlib v0.9.6.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={number of voters},
xmin=5.5, xmax=104.5,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={number of elections},
ymin=-20.9, ymax=438.9,
ytick style={color=black}
]
\addplot [semithick, color0]
table {%
10 67
20 19
30 5
40 5
50 1
60 1
70 0
80 0
90 2
100 1
};
\addlegendentry{0}
\addplot [semithick, color1]
table {%
10 384
20 228
30 194
40 176
50 170
60 162
70 164
80 160
90 155
100 152
};
\addlegendentry{1}
\addplot [semithick, color2]
table {%
10 340
20 418
30 365
40 338
50 284
60 274
70 266
80 236
90 233
100 227
};
\addlegendentry{2-3}
\addplot [semithick, color3]
table {%
10 9
20 135
30 234
40 271
50 327
60 348
70 347
80 382
90 379
100 387
};
\addlegendentry{4-5}
\addplot [semithick, color4]
table {%
10 0
20 0
30 2
40 10
50 18
60 15
70 23
80 22
90 31
100 33
};
\addlegendentry{6-10}
\end{axis}

\end{tikzpicture}
